AvaTaR: Optimizing LLM Agents for Tool Usage via Contrastive Reasoning

Large language model (LLM) agents have demonstrated impressive capabilities in utilizing external tools and knowledge to boost accuracy and reduce hallucinations. However, developing prompting techniques that enable LLM agents to effectively use these tools and knowledge remains a heuristic and labor-intensive task. Here, we introduce AvaTaR, a novel and automated framework that optimizes an LLM agent to effectively leverage provided tools, improving performance on a given task. During optimization, we design a comparator module to iteratively deliver insightful and comprehensive prompts to the LLM agent by contrastively reasoning between positive and negative examples sampled from training data. We demonstrate AvaTaR on four complex multimodal retrieval datasets featuring textual, visual, and relational information, and three general question-answering (QA) datasets. We find AvaTaR consistently outperforms state-of-the-art approaches across all seven tasks, exhibiting strong generalization ability when applied to novel cases and achieving an average relative improvement of 14% on the Hit@1 metric for the retrieval datasets and 13% for the QA datasets. Code and dataset are available at https://github.com/zou-group/avatar.

==> 1.intro_old.tex <==

\jure{
See my new abstract. \\
Notice that However is now different.\\
Notice that KG retrieval is not explicitly mentioned --- we abstract it put and say that the task we are solving is automatically coming up with a prompt.\\
I don't understand the "inductive" part. I think we don't need it. We can skip it and focus on optimization part.
}


\jure{We need to rewrite the introduction like this:\\ \\
Paragraph 1: LLMs are important, agents can do cool stuff, and can use tools (we need to define what a tool is) to be able to perform hard tasks like complex question answering that require multiuple steps of reasoning and retrival of many different pieces of knowledge.\\ \\
Paragraph 2: building such systems is hard because it requires first building the tools, and then engineering a complex prompt that "teaches" the LLM how to effectively decompose a given task, then use the tools, and effectively combine their outputs to synthesize the answer. This is very hard manual work that requires lots of manual labor and lots of trial-and-error before a satisfactory prompt is engineered. ((note there are 3 steps here: given (Q,A), step 1: decompose Q, step 2: use tools, step 3: combine the outputs and synthesize the answer.0)\\ \\
Paragraph 3: An alternative solution would be to develop a system that would take a training set of (query, answer) pairs and would automatically learn how to: (1) decompose the Q into a plan; (2) use the tools; (3) synthesize the outputs into an answer. An important component here is that the system needs to be able to use primitive tools and combine them to solve a more complex tasks. Having a solution like this would be important because it would save a lot of time and would lead to more accurate RAG systems. \\ \\
Paragrap 4: Here we ...
}

Knowledge bases (KBs) serve as explicit and grounded sources of knowledge~\cite{wikipedia, stark, vg, flickr30k_ent, primekg}, complementing the world knowledge encoded in the model parameters~\cite{rag, realm, ra_cm3}.
% \vassilis{add references here for KG}
On top of these KBs, information retrieval aims to extract knowledge that is highly relevant to a user's query, addressing diverse user requests. 
The retrieval tasks provide informative context and are fundamental to various systems, such as dialogue~\cite{PCKW21}, question-answering~\cite{KarpukhinOMLWEC20, QuDLLRZDWW21}, and recommender systems~\cite{RajputMSKVHHT0S23}.


%%%%%% PROBLEM WE WANT TO SOLVE %%%%%%
\xhdr{Problem setting: Autonomous agent for KB retrieval} On these retrieval tasks, autonomous agents empowered by large language models (LLMs) have emerged as a promising direction~\cite{llm4ir}. 
These LLM-based agents~\cite{shi2024ehragent, check_n_try} exhibit impressive problem-solving abilities, such as reasoning~\cite{Wei0SBIXCLZ22, WSLCNCZ23, react, tot}, planning~\cite{HuangAPM22, zheng2023outline, HuangXXCLFZTMCS22, abs-2309-09971}, and using external tools such as knowledge base APIs, to assist the information retrieval process~\cite{shi2024ehragent, toolformer, autogen, chameleon, HuangAPM22, camel}. 
% For example, the retrieval process by an agent can involve a sequence of actions, include accessing, interacting with, and reasoning over data from knowledge bases.
Moreover, as real-world retrieval systems often face diverse user queries, agents are required to effectively generalize to \textit{unseen} queries through inductively learning general principles from seen queries.


%%%%% WHY HASN'T IT BEEN SOLVED / WHY IS IT HARD %%%%%
\xhdr{Limitations and challenges} However, previous LLM-based approaches~\cite{agentbench,prompt_agent,react,dsp} generally focus on non-inductive applications of agents. Specifically, these methods typically model the retrieval tasks for different queries as isolated prompting processes with LLMs, which can prove brittle and often underperform in terms of retrieval accuracy.
We provide a demonstration of such failure cases in Figure~\ref{fig:non_inductive}, where the action sequence generated by ReAct~\cite{react} leads to trivial and misleading solutions. 
Furthermore, while existing research~\cite{llm_as_opt,self_debug, llm_as_opt,prompt_agent, RLPrompt, human_prompt_eng,retroformer, agent_optimizer} widely explores LLMs as optimizers to enhance task performance, it fails to exhibit generalization and the ability to conduct inductive retrieval in the optimization process.
% , such as optimizing mathematical problems~\cite{llm_as_opt,self_debug,optimus,llm4bo}, prompts~\cite{llm_as_opt,prompt_agent, RLPrompt, human_prompt_eng,retroformer}, and function libraries~\cite{agent_optimizer}, they do not consider the generalization ability explicitly in the optimization process. 
Nonetheless, directly improving generalization ability of agents on specific tasks is extremely challenging as most of the state-of-the-art LLMs~\cite{chatgpt,claude3} are closed-source, which restricts the ability to capture task-specific inductive bias within the model parameters and generalize to new instances. 

% In this context, our goal is to optimize the agent retriever for efficient and inductive retrieval on user queries.
% While previous works have widely explored LLMs as optimizers for optimizing mathematical problems~\cite{llm_as_opt, self_debug,optimus,llm4bo} and prompts~\cite{llm_as_opt,prompt_agent, RLPrompt, human_prompt_eng}, optimizing agents presents a more significant challenge due to the multistep reasoning and actions involved. 
% Existing efforts in agent optimization, such as learning a retrospective model for agent prompt tuning~\cite{retroformer} and searching for optimal functions for the agent system~\cite{agent_optimizer}, provide initial solutions. 

% Analogous to \textit{model overfitting}, where models with a larger number of parameters than the size of the data may perform well on training data but not on testing data, agents can become overspecific to certain instances while being misleading and inapplicable to others. We refer to this phenomenon as \textit{agent overfitting}. For example, as depicted in Figure 1(b), the agent checks if each query contains the word ``fashion'' based on received feedback to retrieve correct items. Such agents with systematic flaws do not generalize well to other queries, resulting in poor retrieval performance.

%%%%%%%%% HOW DID WE DO IT %%%%%%%%%%%
\xhdr{Our work: \underline{A}gents for \underline{I}nductive \underline{R}etrieval (AIR)} To address the challenges, we introduce \methodt, a novel framework that optimizes an \subt's action sequence to perform inductive retrieval on KBs. 
\jure{This last sentence is too narrow. We don't need to explicitly say "a novel framework that optimizes an \subt's action sequence to perform inductive retrieval on KBs.". We can say "an automatic framework that optimizes an LLM
agent to be able to effectively use the provided tools and improve its performance6
on a given task."  You can then say:  We demonstrate our framework on  "inductive retrieval on KBs"}

\begin{itemize}[leftmargin=*]
\item \xhdr{Optimization phase} As shown in Figure~\ref{fig:overview}, the core of our optimization framework is a \core module that generates feedback to improve the generalization ability of \subt's action sequence. 
Specifically, the \core takes positive and negative query samples on which the current agent performs well and poorly, respectively, to identify systematic errors exhibited by the agent. 
Unlike case-by-case feedback, the \core provides a more holistic and inductive perspective from the batch of positive and negative instances, which encourages the agent to identify key flaws in its action sequence that lead to suboptimal performance.

\item  \xhdr{Deployment phase} The iterative optimization through our \method framework refines \sub for inductive knowledge extraction, allowing direct application to novel user inquiries in the deployment time. Figure~\ref{fig:inductive} shows the \subt's action sequence after optimizing on training queries, demonstrating the precise extraction of multifaceted attributes and the implementation of a sophisticated scoring system. Moreover, it demonstrates the strategic combination of different scores, determined by the learnt coefficients, ensuring accurate and comprehensive retrieval.
% \vassilis{word choice} 
\end{itemize}

%%%%%%%%% HOW WELL DOES IT PERFORM %%%%%%%%%%%
\xhdr{Experimental evaluation} We conduct extensive experiments on four KB retrieval datasets. The retrieval task are of high complexity due to the multimodal data on the KBs, including textual attributes, images, and relational information. 
We compare the performance of \method with state-of-the-art methods, where \method achieves an average relative improvement of 12.7\% on the Hit@1 metric. Finally, we provide insights and analyze the evolution of agents during the optimization process.

%%%%%%%%% WHAT ARE OUR KEY CONTRIBUTIONS %%%%%%%%%%%
Our key contributions are:
\begin{itemize}[leftmargin=*]
    \item We introduce a novel framework, \methodt, that optimizes an \sub for inductive retrieval on KBs. Our approach involves a \core module that samples diverse instances to provide holistic feedback, improving the agent's ability to generalize to unseen queries. 
    \item We demonstrate that \method significantly outperforms existing state-of-the-art methods on KB retrieval tasks, where the improvements are supported by a detailed analysis on agent evolution.
\end{itemize}




% they focus on optimizing the agents case by case, while 
% as the optimization space of previous works is limited to prompts and function libraries, the agents could be nonoptimal in other reasoning-intensive aspects, such as orgnizing the action sequences and 
% they lack the capability to optimize agents involving complex action sequence and high-level strategies, which are crucial for retrieval performance as discussed above.
% Besides the extended complexity of the optimization space, agent retrievers are required to gain a deep understanding of
% complex knowledge  and unseen query types. 
% The challenge here can be further elevated when dealing with complex queries involving multimodal or heterogeneous data in the knowledge bases. 
% Thus, the agent retrievers require a deep understanding of the knowledge bases and effective generalization to unseen user queries.
% optimizing agent retrievers is challenging since large-scale knowledge bases can only be partially observed during retrieval. 
% Retrieving information is hard because the optimal solution is always case by case, or knowledge base by knowledge base. Knowledge base retrieval have its own properties to consider. 
% One can consider agents in this case as doing sparse retrieval, dense retrieval, conducting string matching or comparing embedding similarity, or even experts in certain domain.

% \begin{figure}[t]
%     \centering
%     \includegraphics[width=0.96\textwidth]{figs/inductive_example2}
%     \caption{
%     \vassilis{The figure is a bit too overloaded. We need to simplify. a) Consider shortening the sentences even if the text does not 100\% correspond to the prompt. b) Put our solution in the bottom and the baseline in the top c) There is an arrow from the top figure pointing to the bottom figure.}
%     Illustration of inductive vs. non-inductive retrieval on product searches.
%     (a) 
%     Inductive retrieval: We optimize the \sub agent and improve its retrieval strategies by leveraging data from training queries, facilitating the application of inductive learning for a wide array of queries. This enables the agent to generalize and apply its refined retrieval process effectively to unseen testing queries.
%     (b) Non-Inductive retrieval: For a specific query, here presents an isolated retrieval process lacking inductive learning, which results in suboptimal retrieval actions.}
%     \label{fig:example}
%     \vspace{-10pt}
% \end{figure}


==> 2.related_old.tex <==
\section{Related Work [TO UPDATE]}
\label{sec:related}

\begin{table}[t]
  \centering
  \caption{Comparison between \method with other agent methods.}
  \label{tab:setting}
  \begin{tabular}{lccccc}
    \toprule
     & {Self-improvement} &  {Memory} & Automatic holistic prompt generation\\
     \midrule
     ReAct~\cite{react}
     & \textcolor{Red}{\ding{55}} 
     & \textcolor{Red}{\ding{55}} 
     & \textcolor{Red}{\ding{55}}\\
     Self-refine~\cite{self_refine}
     & \textcolor{LimeGreen}{\ding{52}}
     & \textcolor{Red}{\ding{55}}
     & \textcolor{Red}{\ding{55}}\\
     Reflexion~\cite{reflexion}
     & \textcolor{LimeGreen}{\ding{52}}
     & \textcolor{LimeGreen}{\ding{52}}
     & \textcolor{Red}{\ding{55}}\\
     \method (Ours)
     &\textcolor{LimeGreen}{\ding{52}}
     &\textcolor{LimeGreen}{\ding{52}}
     &\textcolor{LimeGreen}{\ding{52}}\\
    \bottomrule
  \end{tabular}
\end{table}

\xhdr{Agent Optimization}
In the field of improving LLM agents, previous works have modified the parameters of LLMs through instruction tuning to enhance agent capability~\cite{agent_tunning, toolllm} or generated better prompts through iterative prompt tuning~\cite{llm_as_opt, retroformer,prompt_agent}. 
Recently, \citet{agent_optimizer} conduct agent training by iteratively updating the agents' functions according to the execution history.  
However, these methods do not optimize the inductive ability of agents in their framework explicitly.
% While optimized agents may perform well on training data or similar instances, it is not clear if they can maintain this performance on unseen instances.
Such an ability to generalize from specific examples to novel situations is essential for real-world applications.
In this context, previous attempts has explored inductive reasoning in LLMs~\cite{inductive_reason, hypothesis_search}.
However, improving agents' inductive ability during optimization has received less attention, which can significantly hinder effective agent optimization. 
To address this, we introduce a novel framework inspired by contrastive reasoning to conduct inductive retrieval, focusing on knowledge base retrieval as the downstream task. 
The task poses a significant challenge for agent optimization compared to previous works, due to the complexity of action sequences and the additional dependency on the knowledge base.

\xhdr{LLM Agents for Information Retrieval} 
Recent research has been leveraging the remarkable language understanding and reasoning abilities of LLMs~\cite{Wei0SBIXCLZ22,tot,got,reflexion,react} to improve Information Retrieval (IR) systems,
through pretraining~\cite{realm, qagnn, retro,ioannidis2022graph-aware-bert}, reranking~\cite{llm_reranker, reranking_agents}, and prompting techniques~\cite{dsp,g_retriever}. 
See \citet{llm4ir} for a comprehensive survey. 
In the IR systems, retriever module serves as a key component that directly influences the performance of downstream tasks, such as retrieval-augmented generation~\cite{rag, webgpt,memgpt} and knowledge-intensive question answering~\cite{check_n_try, yang2018hotpotqa}. 
For complex tasks such as retrieving from knowledge bases, previous works regard LLMs as agents that can interact with the environments~\cite{agent_ai,shi2024ehragent,chameleon,autogen,HuangAPM22,camel,dsp,react,self_debug,self_refine} and leverage external tools~\cite{hugginggpt, gorilla,ZhuangYWSZ23,toolformer,triad,agent_ai}. For example, ReAct~\cite{react} conducts reasoning and action in an interleaved way, which retrieves information from Wikipedia to support reasoning. 
EHRAgent~\cite{shi2024ehragent} is designed for EHR question-answering, capable of retrieving relevant clinical knowledge through a structured tool-use planning process and an interactive coding mechanism.
However, these LLM agents mostly operate on individual cases in isolated workflows, where inductive knowledge cannot be transferred from one case to another. 
This lack of transferability negatively impacts applications where inductive knowledge is crucial, such as understanding the patterns in previous queries or data relationships in knowledge bases for precise user recommendations.

% However, the obstacle that affects agent performance can go beyond the design of function library and prompts. 
% For example, the agent can be overfit on some instances such as those used to generate feedback to optimize the agent in the previous optimization step. 

% \xhdr{LLM Agents for Program Synthesis}
% EHRAgent~\cite{shi2024ehragent}, Self-debugging~\cite{chen2023teaching}, \cite{haluptzok2022language}, ReAct~\cite{yao2022react}, Agent AI~\cite{durante2024agent}
% Outline-then-details~\cite{zheng2023outline}
% \citet{ni2023lever} rerank program by trained verifiers to determine the correctness of a program.
% Program-aided LM\cite{gao2023pal} Multi-step reasoning and tool use~\cite{paranjape2023art}

% \xhdr{Multi-Agent Systems}

% Multi-agent systems for constructing knowledge graph~\cite{abs-2312-03022}

% Recent works include simulating interactive environments~\cite{generative_agents, cgmi}, role playing~\cite{camel, dylan}, reasoning~\cite{multiagent_debate, abs-2305-19118, dylan}, demonstrating the huge potential of multi-agent systems in handling complex real-world scenarios.

% LLM as a planner~\cite{chameleon}; 
% Decompose task to choose tools~\cite{ruan2023tptu} 

% \citet{wang2023unleashing} use LLMs to generate prompts for agents in response to a task query. \cite{agentverse} select a fixed number of agents from a set of manual prompt candidates via an additional LLM during each round of discussion. 

==> 3.formulation_old.tex <==

\section{Formulation: Knowledge Base Retrieval using LLM Agents}
\label{sec:formulation}



\xhdr{Knowledge Base} We define a knowledge base (KB) as $\mathcal{K}(\mathcal{E}, h)$, where $\mathcal{E}$ is a set of entities along with their associated knowledge and $h$ represents the KB schema. 
 % to be retrieved \vassilis{Unclear: do not define based on the function (retrive)} from
The entities can vary in nature; for example, they can be e-commerce products, a set of protein and drug entities in a biomedical database, or everyday objects in a visual recognition system.
The schema $h$ describes the format and structure of the KB, dictating how the knowledge is organized and accessed.
% \vassilis{why you do not call these entities instead of units for retrieval} 

The knowledge associated with these entities can be in free-form formats and modalities. For example, the knowledge can be relational, such as complementary relationships between products; textual, like drug descriptions; or visual, represented by images of objects. Moreover, it can be a combination of multiple modalities, \eg integrating relational and textual data, for a comprehensive view of the knowledge. 

\xhdr{Retrieval Tasks} 
For a user query $q$, the task of KB retrieval involves identifying a relevant subset from entities $\mathcal{E}$. 
% \vassilis{overall try to be more concise e.g. you defined KB early on but you do not use.}
We define the training dataset as \(\mathcal{D} = \{(q_i, \mathcal{Y}_i)\}_{i=1}^m\) and the testing dataset as \(\mathcal{D}' = \{(q'_i, \mathcal{Y}'_i)\}_{i=1}^n\), where $\mathcal{Y} \subseteq \{0,1\}^{|\mathcal{E}|}$ and $\mathcal{Y}' \subseteq \{0,1\}^{|\mathcal{E}|}$ are the ground truth entities within the KB that satisfy the queries. The retriever model is denoted as 
\begin{equation}
    \mathcal{M}_{\theta}: (q, \mathcal{K}) \rightarrow v \in \mathbb{R}^{|\mathcal{E}|}
    \label{eq:equation}
\end{equation}
where each output element \(v_k\) is a numeric value indicating the relevance score of the \(k\)-th unit with respect to the input query. 
$\theta$ represents the model state or parameters. 
The retriever model infers the intent and context of a query, and then searches through the KB to find entities that best match the query's requirements. 
The effectiveness of retrieval is assessed using metrics such as mean reciprocal rank (MRR), denoted as $\mathcal{R}: \mathbb{R}^{|\mathcal{E}|} \times \{0,1\}^{|\mathcal{E}|} \rightarrow \mathbb{R}$, which compares the ranking of entities in $s$ against the ground truth.

\xhdr{Agent Retriever} An agent retriever is an instance of the retrieval model $\mathcal{M}$ described in Equation~\ref{eq:equation}.
It computes score vectors through a sequence of actions \(\alpha = \{\alpha_1, \alpha_2, \ldots, \alpha_L\}\). 
These actions belong to an action space $\mathcal{A}$ that comprises various API tools~\cite{retroformer,agent_optimizer}, detailed in Section~\ref{sec:exp}. For example, the actions can be accessing data using knowledge APIs, embedding text or images into vector representations by tools for data processing, and classifying or extracting information driven by language models.
Each action \(\alpha_{\ell}\) ($\ell > 1$) in the sequence may selectively incorporate intermediate results generated by previous actions \(\{\alpha_1, \ldots, \alpha_{\ell-1}\}\). 
The ultimate goal of the agent retriever is to identify an optimal sequence of actions that can effectively perform retrieval tasks for a diverse set of user queries in the dataset \(\mathcal{D}'\). 
\begin{equation}
\quad \max_{\alpha} \mathcal{R}(\mathcal{M}_{\alpha}(q'_i, \mathcal{K}), \mathcal{Y}'_i) \quad \text{for each} \quad (q'_i, \mathcal{Y}'_i) \in \mathcal{D}'
\label{eq:objective}
\end{equation}

% \begin{figure}[t]
%     \centering
%     \includegraphics[width=1\textwidth]{figs/ours}
%     \caption{\textbf{Optimized Retrieval Actions (Ours).} We optimize the \sub agent and improve its retrieval strategies by leveraging data from training queries, such as comprehensive query attribute parsing and scoring system, facilitating the application of inductive learning for a wide array of queries. This enables the agent to generalize and apply its refined retrieval process effectively to unseen testing queries.}
%     \label{fig:inductive}
%     \vspace{-10pt}
% \end{figure}

\section{Problem Analysis and Intuitions}

Next, we delve into an analysis of the retrieval problem that lays the groundwork and sheds light on our optimization framework.

% This introduces why naive methods fail
\begin{itemize}[leftmargin=*]
    \item \xhdr{Zero-shot / Interactive Prompting} 
    % Given a test query, a straightforward approach to conduct retrieval is to 1) construct prompts directly from the user query, KB schema, and potential actions, \ie $(q, h, \mathcal{S})$, and then 2) 
    A straightforward approach to conduct retrieval is to directly prompt the agent to generate the action sequence, which is used to compute the retrieval scores. However, in a zero-shot setting, LLM agents often face difficulties in generating outputs that are both correct and relevant~\cite{agentbench, zheng2023outline}. 
    In previous studies such as ReAct~\cite{react} and DSP~\cite{dsp}, researchers have implemented step-by-step interactive prompting with LLMs to enhance reasoning. Despite these advances, these systems are inherently unable to learn and apply general retrieval principles that would enable broader generalization.
    % \vassilis{They do not generate an action sequence but rather a single action. Or not?}
    
    % this links to that getting feedback is non-trivial 
    \item \xhdr{Few-shot Prompting} The limitations of zero-shot performance have led to the exploration of few-shot or in-context prompting methods~\cite{agentbench,voyager}, which use manually crafted few-shot examples, \eg human-designed action sequences. While these few-shot examples offer guidance for retrieval, they may not always be optimal in design or relevant with unseen queries, which may not generalize well in the applications.
    
    % However, crafting specific and insightful demonstrations for the agent to follow can be a demanding and time-consuming task~\cite{agent_optimizer}, which is further made complicated considering the diverse nature of user queries.
    
    % \item \xhdr{Interactive Prompting} 
    % To improve the action sequence for each test query, previous works like ReAct~\cite{react} and DSP~\cite{dsp} have employed step-by-step interactive prompting with LLMs. They iteratively generate outputs or thoughts based on the current action sequence to determine the next action. 
    % However, these approaches may face challenges due to the limited context length of LLMs, which can restrict the amount of information that can be processed and stored for each step. As a result, the effectiveness of the interactive prompting is constrained, which may impact the overall performance of the retrieval system. \vassilis{The way it is written it seems that the main challenge we solve is the limited context length. Explain the limitation of these approaches with respect to our work.} \vassilis{Most of these approaches are not learnable, different than ours. The agent optimization framework in this work allows to improve with these methods.} \vassilis{Call it out also earlier in the doc}
    
    % However, due to the extensive size of KBs, the intermediate results, such as text and relational data, can be of vast amount, which can easily exceed the limited context size. Additionally, generating customized solutions for each test query is costly and time-consuming, which may not be practical in the real settings.
\end{itemize}

The observations underscore the persistent gaps in LLM retrieval systems, summarized as follows:

\begin{intuition}
Previous approaches to KB retrieval that utilize zero-shot, interactive, or few-shot prompting with LLMs have primarily focused on non-inductive retrieval, which lacks the ability to generalize and outperform on diverse and unseen queries. This focus has resulted in significant limitations in retrieval accuracy.
\end{intuition}

% \vassilis{Motivate this more when you present the bullets above}
% \textit{The above methods that directly apply LLMs or use improved prompting techniques for each test query often result in insufficient retrieval performance or face challenges of feasibility.}

To clarify, the above retrieval methods process each query independently, leading to a lack of inductive modeling. 
We refer to \textit{inductive modeling} as the essence of deriving general principles from previously seen data and applying these principles to unseen situations. However, the lack of this inductive modeling limits the broader applicability of autonomous retrieval systems, which is crucial in the real world. Nevertheless, exhibiting the generalization ability faces several challenges:


\begin{itemize}[leftmargin=*]
    \item \xhdr{Close-source Model Access} Fine-tuning model parameters has become a common approach to capture the inductive bias of specific tasks. However, current state-of-the-art LLMs~\cite{gpt4, claude3} are mostly close-source, meaning that they do not provide access to model parameters that can be fine-tuned on the KB retrieval tasks to generate effective action sequences on new queries.
    
    \item \xhdr{Inadequate Optimization} 
    Another approach to enable inductive retrieval is learning an action sequence from training data that can be directly applied to test queries. For example, OPRO~\cite{llm_as_opt} proposes a paradigm that optimizes solutions generated by LLMs by generating new solutions from prompts containing past solutions and their optimization scores. However, due to the dependency on KBs, the pairs of action sequence and their numerical scores lack a clear direction for agent improvement, leading to ambiguity in refining retrieval strategies. Other approaches~\cite{self_debug, self_refine, reflexion} generate feedback from executing on specific instances (unit tests) provides explicit directions for improvement, but can they easily result in non-generalizable solutions, where agents become overspecific to certain instances and fail to generalize to others. 
    We validate the above issues in the experimental study.
\end{itemize}

\textbf{Key Intuition 2:} \textit{Improving agents' ability in inductive modeling remains an open challenge since the state-of-the-art LLMs are close-source and current optimization frameworks are inadequate and can easily result in non-generalizable solutions.}

Motivated by the above analysis, the goal of this work is to optimize agents for inductive retrieval, enhancing the generalization of the retrieval process to unseen queries.



==> 4.model_old.tex <==
\section{Our Method: Optimizing Agents for Tool-Assisted Retrieval [UPDATING]}
\label{sec:method}


\begin{figure}[t]
    \centering
    \includegraphics[width=1\textwidth]{figs/case.pdf}
    \caption{\textbf{Illustration of the \sub and \core during optimization.} Best viewed in color. Delving deeper into Figure~\ref{fig:overview}, the illustration demonstrates: (a) the development of prompts for the \coret, outlining the task with examples of positive and negative queries, and (b) feedback from the \coret, providing insights that guide the \sub to generate more generalizable actions.}

    \label{fig:case}
\end{figure}

Our optimization framework, \methodt, introduces a novel approach to knowledge base (KB) retrieval using LLM agents. 
In Table~\ref{tab:setting}, we highlight three critical aspects of our approach: self-improvement mechanisms, memory construction, and the capability to conduct inductive modeling. We compare \method with prevailing agent framework~\cite{react, reflexion, self_refine} to underscore the advancements our work offers.

We firstly introduce the two LLM components in \methodt: an \sub $\mathcal{M}_a$ and a \core $\mathcal{M}_c$. 

\xhdr{Actor} The actor, $\mathcal{M}_a$, is responsible for generating actions based on the current state, and conducting the action sequence to retrieve relevant information from the KB. For clarity, we denote the action sequence at iteration $t$ as $\alpha^{(t)}=\{\alpha^{(t)}_1,\alpha^{(t)}_2,\ldots\}$ (\cf notation in Section~\ref{sec:formulation}). Specifically, at step $t$, $\mathcal{M}_a$ takes prompts including the current action sequence $\alpha^{(t)}$ as inputs, and outputs the updated actions sequence $\alpha^{(t+1)}$. 
The updated actor sequence will navigate the vast and complex structure of the KB and retrieve relevant information based on user query.
%  \vassilis{use consistently either actions or thoughts. Or define the difference.}

\xhdr{Contrastor} The \coret, $\mathcal{M}_c$, plays a key role in our optimization framework, which provides feedback for the \sub $\mathcal{M}_a$ to promote inductive retrieval. 
As shown in Figure~\ref{fig:overview}, t, instead of generating feedback on individual instances through self-explanation and self-reflection, \core aims to identify systematic flaws that hinder the generalization of the current action sequence. 
To realize this goal, \core first constructs positive and negative queries from the evaluation phase. Specifically, positive instances are queries from the training set where the \sub performs well, and negative instances are queries where the \sub underperforms. We measure the performance of the ranking results for each query via metrics such as Mean Reciprocal Rank (MRR). In each iteration, \core randomly samples a mini-batch with an equal number of positive and negative queries, where the total batch size $b$ is a hyperparameter.

% \vassilis{This is a major contribution of this work let highlight it better} 
%  \vassilis{Here, we can have hard and soft negatives where the agent outperforms by a lot and marginally outperforms. This could help achieve even better results. Let's discuss further.}

As shown in Figure~\ref{fig:case} (a), we prompt the contrastor to contrast patterns between the positive and negative queries, and simulate the retrieval processes on these two group of queries separately to identify any discrepancies in the action sequence logic. 
As demonstrated in Figure~\ref{fig:case} (b), the \core notes that negative queries often contain complex product feature descriptions. This observation indicates that the \subt’s action sequence may not adequately capture product relevance. Informed by this feedback, \sub updates its action sequence to more effectively account for these nuances, improving performance across a broad set of queries.


\xhdr{Key insights of \coret} Drawing an analogy from the training of deep neural networks, where extremely small batch sizes can introduce significant noise in gradient estimates and high variance in model updates, we adopt a similar batching strategy for the \coret. By sampling multiple queries from the training dataset as a ``batch'', our method allows the \core to extract a robust ``gradient'' to update the \subt. To highlight, the contrastive analysis is particularly effective for inductive modeling as it focuses on identifying and rectifying systemic flaws affecting a wide range of queries. As a result, the \sub develops a more generalized action sequence, which is not only tailored to individual instances but also outperforms across a broader array of queries, thereby enhancing overall retrieval performance.

\xhdr{Other feedback types}
% \vassilis{ Can we highlight more this and the next section as contributions}
In addition to the feedback provided by the contrastor, our framework incorporates two additional types of feedback to enhance the validity and efficiency of the \subt:
% , which are commonly implemented by previous works~\cite{reflexion,llm_as_opt}.

\begin{itemize}[leftmargin=*]
    \item Validity check: This feedback is triggered internally during the execution of each action. It ensures the validity of the \subt's actions, such as verifying the proper use of function calls and confirming that the final score vector returned by the \sub is of the correct size. 
    \item Timeout Error: To preclude inefficient action sequences that may stall the \subt, we implement a timeout mechanism that triggers an error when processing exceeds a threshold. This error prompt the \sub to use more efficient strategies, such as eliminating redundant operations.
    \item Developer performance: As an augmentation following previous works~\cite{llm_as_opt, reflexion}, we assess the \subt's performance on a small set of holdout queries from the training set (if the \sub passes both the validity check and timeout test). We use Mean Reciprocal Rank (MRR) metric and Hit Rate for this evaluation. This feedback guides the optimization on retrieval accuracy.
    
\end{itemize}

\xhdr{Memory Storage}
During optimization, we utilize a memory bank with both short-term and long-term memory, inspired by human decision-making processes, where human tends to address current problems by analyzing the current situation and referencing past experiences.
The short-term memory includes the current action sequence paired with the corresponding feedback. The long-term memory stores tuples of action sequences, feedback from the contrastor, and developer performance. To manage the context size input to the actor at each iteration, we retain only the top-$k$ action sequences with the best performance. Therefore, this memory bank enables the \sub to learn from both immediate feedback and historical data, with an emphasis on the contrastor's role in providing guidance for inductive retrieval. 

\xhdr{Inference} 
At inference, the optimized action sequence, with its inductive modeling ability, will be applied to retrieve relevant entities from the KB for a diverse set of user queries. 


% Through iterative optimization, our framework \method fine-tunes the \subt's action sequences, ensuring they are not only effective on the training queries but also adaptable to new, unseen queries. This process is facilitated by the continuous interaction between the \sub and the contrastor, with the latter providing constructive feedback that guides the \subt's evolution. As a result, \method is capable of optimizing actors for inductive modeling, significantly enhancing the overall effectiveness of the retrieval system.

% As illustrated in Figure 2, our proposed optimization framework \method is comprised of two language model components: a LLM agent, which generates and conducts action sequence, denoted as $\mathcal{M}_a$ and a contrastor LLM, denoted as $\mathcal{M}_c$.

==> tables/2p_case.tex <==

\begin{tabular}{cccccc}
\toprule[1.2pt]
\textbf{Case} & \textbf{Head}&&\textbf{Intermediate entity}&&\textbf{Tail}\\
&(Groundtruth)&&(Top 3 prediction)&&(Prediction)\\
\hline
Interpretability&{Elmira(U.S. City)}&{\textit{location in}}&{U.S.}, {Canada},{UK}&\textit{in country}&Davidson College\\ 
\midrule
\multirow{2}{*}{\makecell[c]{All-direction\\Reasoning}}&\multirow{2}{*}{\textit{Salt}(2010 film)}&\multirow{2}{*}{\textit{has subject}}&\textbf{\textcolor{orange}{CIA}}, Espionage, PTSD&\textit{employs}&George Bush\\ \cmidrule{4-4} \cmidrule{6-6}
&&&\textcolor{red}{Serial killer}, Espionage, PTSD&\textit{(masked)}&-\\
\bottomrule[1.2pt]
\end{tabular}





==> tables/3p_case.tex <==
\small
\begin{tabular}{
p{2.2cm}<{\centering}
p{1.4cm}<{\centering}
p{2.0cm}<{\centering}
p{1.4cm}<{\centering}
p{2.1cm}<{\centering}
p{1.5cm}<{\centering}
p{1.8cm}<{\centering}
}
\toprule[1.2pt]
\textbf{Head}&&\textbf{Intermediate 1}&&\textbf{Intermediate 2}&&\textbf{Tail}\\
(Ground truth)&&(Back-queried)&&(Back-queried)&&(Assumed fact)\\
\hline
\multirow{3}{*}{TV5 (TV network)}&\multirow{3}{*}{\textit{\makecell[c]{leader-\\title}}}&President&\multirow{3}{*}{\textit{\makecell[c]{company-\\with-title}}}&Verizon&\multirow{3}{*}{\textit{\makecell[c]{region-\\in}}}&New York\\
&&President&&eBay&&California\\
&&President&&Ford Motor&&Michigan\\
\hline
\multirow{3}{*}{Priyanka Chopra}&\multirow{3}{*}{\textit{gender}}&Female&\multirow{3}{*}{\textit{\makecell[c]{risk-\\ factors}}}&Hypothyroidism&\multirow{3}{*}{\textit{\makecell[c]{risk-\\factors}}}&Depression\\
&&Female&&Cirrhosis&&Peritonitis\\
&&Female&&Cirrhosis&&Liver failure\\
\hline
\multirow{5}{*}{Clarinet}&\multirow{5}{*}{\textit{role}}&Paquito D'Rivera&\multirow{5}{*}{\textit{Profession}}&Musician&\multirow{5}{*}{\textit{\makecell[c]{specialization-\\of}}}&Artist\\
&&Imogen Heap&&Singer-songwriter&&Musician\\
&&Harry Shearer&&Author&&Writer\\
\bottomrule[1.2pt]
\end{tabular}


==> tables/benchmark_examples.tex <==

\begin{table}[htbp]
    \resizebox{1.0\textwidth}{!}{
    \begin{tabular}{ccl}
        \toprule
        & \textbf{Target} & \textbf{Example query} \\
        \midrule
        \hline
        \multirow{4}{*}{\amazont} & \multirow{ 4}{*}{\texttt{product}} & \cellcolor{cyan!5} {\textit{Can you help me find a \textcolor{OliveGreen}{push-along} tricycle \textcolor{MidnightBlue}{from Radio Flyer} that's  }}  \\
        & & \cellcolor{cyan!5} {\textit{\textcolor{OliveGreen}{both fun and safe for my kid}?}}  \\
        \noalign{\vspace{0.85ex}}
        &&\cellcolor{cyan!5} {\textit{What are recommended scuba diving weights \textcolor{OliveGreen}{for experienced divers} }}\\
        &&\cellcolor{cyan!5} {\textit{that would \textcolor{MidnightBlue}{fit well with my Gorilla PRO XL waterproof bag}?}}\\
        \noalign{\vspace{0.7ex}}
        \midrule
        \noalign{\vspace{0.7ex}}
        \multirow{ 3}{*}{\magt} & \multirow{ 3}{*}{\texttt{paper}} & \cellcolor{lime!10} {\textit{Search publications \textcolor{MidnightBlue}{by Hao-Sheng Zeng} on \textcolor{OliveGreen}{non-Markovian dynamics}.}} \\
        \noalign{\vspace{0.85ex}}
        & &  \cellcolor{lime!10}\textit{What are some \textcolor{OliveGreen}{nanofluid heat transfer} research papers published by}\\
        & &  \cellcolor{lime!10}\textit{scholars \textcolor{MidnightBlue}{from Philadelphia University}?} \cellcolor{lime!10}\\
        \noalign{\vspace{0.7ex}}
        \midrule
        \noalign{\vspace{0.7ex}}
        \multirow{5}{*}{\primekgt} & \texttt{disease} & \cellcolor{pink!25}\textit{Is my \textcolor{OliveGreen}{constant fatigue} due to conditions \textcolor{MidnightBlue}{related to bartonellosis}?}\\
        \noalign{\vspace{0.85ex}}
        & \multirow{ 2}{*}{\texttt{drug}} &  \cellcolor{pink!25}\textit{Could you provide a list of \textcolor{OliveGreen}{investigational} drugs that \textcolor{MidnightBlue}{interact with }}\\
        && \cellcolor{pink!25}\textit{\textcolor{MidnightBlue}{genes or proteins predominantly active in the epididymal region}?}\\
        \noalign{\vspace{0.85ex}}
        & \texttt{pathway} & \cellcolor{pink!25}\textit{Please find pathways \textcolor{MidnightBlue}{involving the POLR3D gene} \textcolor{OliveGreen}{within nucleoplasm}.}\\
        \noalign{\vspace{0.85ex}}
        & \texttt{gene} & \cellcolor{pink!25}\textit{Which gene on \textcolor{OliveGreen}{chromosome 4} are \textcolor{MidnightBlue}{expressed in multicellular organisms}?}\\
        \bottomrule
    \end{tabular}
    }
    \vspace{2pt}
    \caption{Example queries from \benchmarkt, where \textcolor{MidnightBlue}{relational requirements} and \textcolor{OliveGreen}{textual requirements} from the semi-structured knowledge bases are highlighted.}
    \label{tab:benchmark_examples}
\end{table}

==> tables/benchmark_sources.tex <==


\begin{table}[t]
    \centering
    \resizebox{1.0\textwidth}{!}{
    \begin{tabular}{l|cc}
        \toprule
        & \textbf{relational structure} & \textbf{textual information}  \\
        \midrule
        \multirow{ 2}{*}{\textbf{\amazont}} &  \multirow{ 2}{*}{Amazon Product Reviews} & Amazon Product Reviews\\
        & & Amazon Question and Answer Data  \\
        \textbf{\magt} & ogbn-mag & 	ogbn-papers100M, Microsoft Academic Graph  \\
        \multirow{ 2}{*}{\textbf{\primekgt}}& \multirow{ 2}{*}{PrimeKG}  & \texttt{disease}: Orphanet; \texttt{drug}: DrugBank; \texttt{pathway}: Reactome; \\
        && \texttt{gene}: Ensembl, NCBI Entrez, Uniprot, UCSC, CPDB \\
        \bottomrule
    \end{tabular}
    }
    \hspace{3pt}
    \caption{Sources of relational structure and textual information of the benchmarks}
    \label{tab:sources}
\end{table}


==> tables/benchmark_stats.tex <==

\begin{table}[htbp]
    \centering
    \resizebox{1.0\textwidth}{!}{
    \begin{tabular}{l|rccc}
        \toprule
        & \textbf{\#queries}  & \textbf{\#multi-answer queries} & \textbf{avg. answer length} & \textbf{train / val / test}\\
        \midrule
        \amazont & 9,100 & 7,082 & 17.99 & 0.65 / 0.17 / 0.18\\
        \magt &13,323 & 6,872 & 2.78 &0.60 / 0.20 / 0.20\\
        \primekgt & 11,204 & 4,188 & 2.56 & 0.55 / 0.20 / 0.25 \\
        \bottomrule
    \end{tabular}
    }
    \hspace{3pt}
    \caption{Data statistics on \benchmarkt.}
    \label{tab:benchmark_stats}
\end{table}

==> tables/expert_speed.tex <==
\begin{tabular}{lccccc}
    \toprule
     \multirow{2}{*}{} & \multirow{2}{*}{Batch size} & \multicolumn{4}{c}{Number of experts}\\\cmidrule(l){3-6}
     \multicolumn{1}{l}{} & \multicolumn{1}{l}{}& 2 & 8 & 16 & 32  \\ 
     \midrule
     Pre-training stage 1 & 64 &41.46 & 42.02 & 45.38 & 49.30 \\
     Pre-training stage 2 & 64 &17.37 & 18.83 & 19.78 & 24.09 \\
     Fine-tuning & 64 & 32.41 & 32.91 & 36.46 & 37.47  \\
     Inference & 3072 & 40.54 & 40.54 & 40.54 & 40.54  \\
     \bottomrule
\end{tabular}

==> tables/hit1_table.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{tabular}{@{}ll|p{0.8cm}<{\centering}p{0.8cm}<{\centering}|p{0.8cm}<{\centering}p{0.8cm}<{\centering}p{0.8cm}<{\centering}p{0.8cm}<{\centering}p{0.8cm}<{\centering}p{0.8cm}<{\centering}p{0.8cm}<{\centering}p{0.8cm}<{\centering}p{0.8cm}<{\centering}@{}}
\toprule[1.2pt]
\multirow{2}{*}{Dataset} & \multirow{2}{*}{Model}    & \multirow{2}{*}{Avg}                      & \multirow{2}{* }{\makecell[c]{Avg\\w.o. u}}                               & \multicolumn{5}{c}{In-domain}                                                                                                                                                      & \multicolumn{4}{c}{Out-of-domain}                \\ \cmidrule(l){5-9} \cmidrule(l){10-13}
\multicolumn{1}{l}{} & \multicolumn{1}{l}{}    & \multicolumn{1}{|l}{} &  & \multicolumn{1}{c}{1p} & \multicolumn{1}{c}{2p} & \multicolumn{1}{c}{3p} & \multicolumn{1}{c}{2i} & \multicolumn{1}{c}{3i} & \multicolumn{1}{c}{ip} & \multicolumn{1}{c}{pi} & \multicolumn{1}{c}{2u} & \multicolumn{1}{c}{up} \\ \midrule
\multirow{8}{*}{FB15k-237}& \multicolumn{1}{|l|}{GQE~\cite{hamilton2018embedding}}                                  & 0.103                                      & 0.250                                                & 0.346                   & 0.193                   & 0.145                   & 0.25                   & 0.355                   & 0.086                   & 0.156                   & 0.145                   & 0.151\\
                          & \multicolumn{1}{|l|}{Q2B~\cite{ren2019query2box}}                                       & -                                      & -                                               & -                 & -                    &-                  &-               & -                 & -                  &-                 & -                   & -                 \\
                          & \multicolumn{1}{|l|}{EmQL~\cite{sun2021faithful}$^1$}                                   & 0.219                                 & 0.241                                                & 0.389                           & 0.201                   & 0.154                   & 0.275                   & 0.386                   & 0.101                   & 0.184                           & 0.115                   & 0.165                  \\
                          & \multicolumn{1}{|l|}{BiQE~\cite{kotnis2021answering}}                                   & -                                          & 0.293                                                & 0.439                   & 0.281                   & 0.239                   & 0.333                   & 0.474                   & 0.110                   & 0.177                   & -                       & -                      \\
                          & \multicolumn{1}{|l|}{HypE~\cite{choudhary2021self}}                                       & 0.335                                      & 0.359                                                & 0.572                   & 0.366                   & 0.255                   & 0.399                   & 0.527                   & 0.145                   & 0.246                   & 0.225                   & 0.282                  \\
                          & \multicolumn{1}{|l|}{CQD\footnotesize{(CO)}\normalsize~\cite{arakelyan2021complex}}     & 0.272                             & 0.290                                                & 0.512                   & 0.213                   & 0.131                   & 0.352                   & 0.457                   & 0.146                   & 0.222                   & 0.281                   & 0.132                  \\
                          & \multicolumn{1}{|l|}{CQD\footnotesize{(Beam)}\normalsize~\cite{arakelyan2021complex}}   & 0.290                             & 0.315                                                & 0.512                   & 0.288                   & 0.221                   & 0.352                   & 0.457                   & 0.129                   & 0.249                   & 0.284                   & 0.121                  \\ \cmidrule{2-13}
                          & \multicolumn{1}{|l|}{\method} & \\\midrule%0.312                                      & 0.334                                                & 0.455                   & 0.306                   & 0.241                   & 0.389                   & 0.513                   & 0.165                   & 0.269                   & 0.264                   & 0.210                                 \\ \midrule
\multirow{8}{*}{NELL995}& \multicolumn{1}{|l|}{GQE~\cite{hamilton2018embedding}}                                    & 0.21                                   & 0.270                                                & 0.311                   & 0.193                   & 0.175                   & 0.273                   & 0.399                   & 0.078                   & 0.168                   & 0.159                   & 0.13                  \\
                          & \multicolumn{1}{|l|}{Q2B~\cite{ren2019query2box}}                                       & 0.254                                      & 0.317                                                & 0.413                   & 0.225                   & 0.173                   & 0.275                   & 0.378                   & 0.105                   & 0.18                   & 0.198                   & 0.178                  \\
                          & \multicolumn{1}{|l|}{EmQL~\cite{sun2021faithful}$^1$}                                   & 0.277                                      & 0.294                                                & 0.456                   & 0.231                   & 0.172                   & 0.331                   & 0.483                   & 0.143                   & 0.244                   & 0.226                   & 0.207                  \\
                          & \multicolumn{1}{|l|}{BiQE~\cite{kotnis2021answering}}                                   & \multicolumn{1}{l}{-}                      & 0.344                                                & 0.587                      & 0.305                   & 0.326                   & 0.371                   & \underline{0.531}                   & 0.103                   & 0.187                   & \multicolumn{1}{l}{-}   & \multicolumn{1}{l}{-}  \\
                          & \multicolumn{1}{|l|}{HypE~\cite{choudhary2021self}}                                       & 0.371                                      & 0.375                                                & \underline{0.618}                      & 0.359                   & 0.312                   & 0.400                   & 0.563                   & 0.143                   & 0.227                   & 0.441                   & \bf 0.278                  \\
                          & \multicolumn{1}{|l|}{CQD\footnotesize{(CO)}\normalsize~\cite{arakelyan2021complex}}     & 0.368                                      & 0.370                                                & \bf 0.667                      & 0.265                   & 0.220                   & \bf 0.410                   & 0.529                   & \underline{0.196}                   & \bf 0.302                   & \bf 0.531                   & 0.194                  \\
                          & \multicolumn{1}{|l|}{CQD\footnotesize{(Beam)}\normalsize~\cite{arakelyan2021complex}}   & \underline{0.375}                                      & \underline{0.385}                                                & \bf 0.667                   & 0.350                   & 0.288                   & \bf 0.410                   & 0.529                   & 0.171                   & 0.277                   & \bf 0.531                   & 0.156                  \\ \cmidrule{2-13}
                          & \multicolumn{1}{|l|}{\method} & \bf 0.398                                      & \bf 0.406                                                & 0.617                   & \bf 0.401                   & \bf 0.367                   & \underline{0.405}                   & \bf 0.546                   & \bf 0.203                   & \underline{0.300}                   & \underline{0.469}                   & \underline{0.270}                  \\ \bottomrule[1.2pt]
\end{tabular}

==> tables/main_table.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{tabular}{@{}llp{0.8cm}<{\centering}p{0.8cm}<{\centering}p{0.8cm}<{\centering}p{0.8cm}<{\centering}p{0.8cm}<{\centering}p{0.8cm}<{\centering}p{0.8cm}<{\centering}p{0.8cm}<{\centering}p{0.8cm}<{\centering}p{0.8cm}<{\centering}p{0.8cm}<{\centering}@{}}
\toprule[1.2pt]
\multirow{2}{*}{Dataset} & \multirow{2}{*}{Model}    & \multirow{2}{*}{Avg}                      & \multirow{2}{* }{\makecell[c]{Avg\\w/o u}}                               & \multicolumn{5}{c}{In-domain}                                                                                                                                                      & \multicolumn{4}{c}{Out-of-domain}                \\ \cmidrule(l){5-9} \cmidrule(l){10-13}
\multicolumn{1}{l}{} & \multicolumn{1}{l}{}    & \multicolumn{1}{l}{} &  & \multicolumn{1}{c}{1p} & \multicolumn{1}{c}{2p} & \multicolumn{1}{c}{3p} & \multicolumn{1}{c}{2i} & \multicolumn{1}{c}{3i} & \multicolumn{1}{c}{ip} & \multicolumn{1}{c}{pi} & \multicolumn{1}{c}{2u} & \multicolumn{1}{c}{up} \\ \midrule
\multirow{8}{*}{\makecell[c]{NELL\\-995}}& \multicolumn{1}{l}{GQE~\tohide{hamilton2018embedding}}                                    & 24.8                                   & 27.0                                                & 41.7                   & 23.1                   & 20.3                   & 31.8                   & 45.4                   & 8.1                   & 18.8                   & 20.0                   & 13.9                  \\
                          & \multicolumn{1}{l}{Q2B~\tohide{ren2019query2box}}                                       & 30.6                                      & 31.7                                                & 55.5                   & 26.6                   & 23.3                   & 34.3                   & 48.0                   & 13.2                   & 21.2                   & 36.9                   & 16.3                  \\
                          & \multicolumn{1}{l}{EmQL~\tohide{sun2021faithful}$^1$}                                   & 27.7                                      & 29.4                                                & 45.6                   & 23.1                   & 17.2                   & 33.1                   & 48.3                   & 14.3                   & 24.4                   & 22.6                   & \underline{20.7}                  \\
                          & \multicolumn{1}{l}{BiQE~\tohide{kotnis2021answering}}                                   & \multicolumn{1}{c}{-}                      & 34.4                                                & 58.7                      & 30.5                   & 32.6                   & 37.1                   & \underline{53.1}                   & 10.3                   & 18.7                   & \multicolumn{1}{c}{-}   & \multicolumn{1}{c}{-}  \\
                          %& \multicolumn{1}{|l|}{HypE~\tohide{choudhary2021self}}                                       & 37.1                                      & 37.5                                                &61.8                      & 35.9                   & 31.2                   & 40.0                   & 56.3                   & 14.3                   & 22.7                   & 44.1                   & \bf 27.8                  \\
                          & \multicolumn{1}{l}{CQD\footnotesize{(CO)}\normalsize~\tohide{arakelyan2021complex}}     & 36.8                                      & 37.0                                                & \bf 66.7                      & 26.5                   & 22.0                   & \bf 41.0                   & 52.9                   & \underline{19.6}                   & \bf 30.2                   & \bf 53.1                   & 19.4                  \\
                          & \multicolumn{1}{l}{CQD\footnotesize{(Beam)}\normalsize~\tohide{arakelyan2021complex}}   & \underline{37.5}                                      & \underline{38.5}                                                & \bf 66.7                   & 35.0                   & 28.8                   & \bf 41.0                   & 52.9                   & 17.1                   & 27.7                   & \bf 53.1                   & 15.6                  \\ \cmidrule{2-13}
                          & \multicolumn{1}{l}{\method} & \bf 39.8                                      & \bf 40.6                                                & \underline{62.5}                   & \bf 40.1                   & \bf 36.7                   & \underline{40.5}                   & \bf 54.6                   & \bf 20.3                   & \underline{30.0}                   & \underline{46.9}                   & \textbf{27.0}                  \\ \midrule
\multirow{8}{*}{\makecell[c]{FB15k\\-237}}& \multicolumn{1}{l}{GQE~\tohide{hamilton2018embedding}}                                  & 23.0                                      & 25.0                                                & 40.5                   & 21.3                   & 15.3                   & 29.8                   & 41.1                   & 8.5                   & 18.2                   & 16.7                   & 16.0                  \\
                          & \multicolumn{1}{l}{Q2B~\tohide{ren2019query2box}}                                       & 26.8                                      & 28.3                                                & 46.7                   & 24.0                   & 18.6                   & 32.4                   & 45.3                   & 10.8                   & 20.5                   & 23.9                   & \underline{19.3}                  \\
                          & \multicolumn{1}{l}{EmQL~\tohide{sun2021faithful}$^1$}                                   & 21.9                                 & 24.1                                                & 38.9                           & 20.1                   & 15.4                   & 27.5                   & 38.6                   & 10.1                   & 18.4                           & 11.5                   & 16.5                  \\
                          & \multicolumn{1}{l}{BiQE~\tohide{kotnis2021answering}}                                   & -                                          & 29.3                                                & 43.9                   & 28.1                   & 23.9                   & 33.3                   & \underline{47.4}                   & 11.0                   & 17.7                   & -                       & -                      \\
                          %& \multicolumn{1}{|l|}{HypE~\tohide{choudhary2021self}}                                       & \underline{33.5}                                      & \bf 35.9                                                & \bf 57.2                   & \bf 36.6                   & \underline{25.5}                   &\bf  39.9                   & \underline{52.7}                   & 14.5                   & 246                   & 22.5                   &\bf 28.2                  \\
                          & \multicolumn{1}{l}{CQD\footnotesize{(CO)}\normalsize~\tohide{arakelyan2021complex}}     & 27.2                             & 29.0                                                & \bf 51.2                   & 21.3                   & 13.1                   & \underline{35.2}                   & 45.7                   & \underline{14.6}                   & 22.2                   & 28.1                   & 13.2                  \\
                          & \multicolumn{1}{l}{CQD\footnotesize{(Beam)}\normalsize~\tohide{arakelyan2021complex}}   & \underline{29.0}                             & \underline{31.5}                                                & \textbf{51.2}                   & \underline{28.8}                   & \underline{22.1}                   & \underline{35.2}                   & 45.7                   & 12.9                   & \underline{24.9}                   & \underline{28.4}                   & 12.1                  \\ \cmidrule{2-13}
                          & \multicolumn{1}{l}{\method} & \bf 33.6                                     & \textbf{35.7}                                                & \underline{47.9}                   & \textbf{32.3}                   & \bf 27.7                   & \textbf{39.8}                   & \bf 53.9                   & \bf 19.0                   & \bf 29.4                   & \bf29.5                   & \textbf{22.5}                                 \\  
\bottomrule[1.2pt]
\end{tabular}

\tohide{
\midrule
\multirow{8}{*}{FB15k}  & \multicolumn{1}{l}{GQE~\cite{hamilton2018embedding}}                                    & 38.4                                      & 40.4                                                & 63.0                   & 346                   & 25.0                   & 51.5                   & 61.1                   & 15.3                   & 32.0                   & 36.2                   & 27.1                  \\
                          & \multicolumn{1}{l}{Q2B~\cite{ren2019query2box}}                                       & 48.3                                      & 48.7                                                & 79.0                   & 41.0                   & 30.0                   & 59.0                   & 71.0                   & 21.0                   & 40.0                   & 61.0                   & 33.0                  \\
                          & \multicolumn{1}{l}{EmQL~\cite{sun2021faithful}$^1$}                                   & 28.7                                      & 31.6                                                & 41.5                   & 25.0                   & 18.8                   & 39.6                   & 50.8                   & 17.6                   & 27.9                   & 16.6                   & 20.7                  \\
                          & \multicolumn{1}{l}{BiQE~\cite{kotnis2021answering}}                                   & \multicolumn{1}{l}{-}                      & \multicolumn{1}{l}{-}                                & \multicolumn{1}{l}{-}   & \multicolumn{1}{l}{-}   & \multicolumn{1}{l}{-}   & \multicolumn{1}{l}{-}   & \multicolumn{1}{l}{-}   & \multicolumn{1}{l}{-}   & \multicolumn{1}{l}{-}   & \multicolumn{1}{l}{-}   & \multicolumn{1}{l}{-}  \\
                          & \multicolumn{1}{l}{HypE~\cite{2021Hyperboloid}}                                       & 51.3                                      & 51.4                                                & 80.9                   & 48.6                   & 36.5                   & 59.8                   & 72.8                   & 20.6                   & 40.6                   & 61.0                   & 41.0                  \\
                          & \multicolumn{1}{l}{CQD\footnotesize{(CO)}\normalsize~\cite{trouillon2016complex}}     & 57.7                                      & 57.9                                                & 92.0                   & 45.0                   & 19.0                   & 80.0                   & 84.0                   & 34.0                   & 51.0                   & 82.0                   & 32.0                  \\
                          & \multicolumn{1}{l}{CQD\footnotesize{(Beam)}\normalsize~\cite{trouillon2016complex}}   & 68.3                                      & 70.9                                                & 92.0                   & 78.0                   & 58.0                   & 80.0                   & 84.0                   & 38.0                   & 66.0                   & 84.0                   & 34.5                  \\ \cmidrule{2-13}
                          & \multicolumn{1}{l}{\method} & \\%60.9                                      & 63.4                                                & 89.2                   & 61.7                   & 46.7                   & 73.6                   & 79.7                   & 38.5                   & 54.7                   & 79.5                   & 24.4                                 \\
}

==> tables/main_table2.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{tabular}{@{}ll|p{0.8cm}<{\centering}p{0.8cm}<{\centering}|p{0.8cm}<{\centering}p{0.8cm}<{\centering}p{0.8cm}<{\centering}p{0.8cm}<{\centering}p{0.8cm}<{\centering}p{0.8cm}<{\centering}p{0.8cm}<{\centering}p{0.8cm}<{\centering}p{0.8cm}<{\centering}@{}}
\toprule[1.2pt]
\multirow{2}{*}{Dataset} & \multirow{2}{*}{Model}    & \multirow{2}{*}{Avg}                      & \multirow{2}{* }{\makecell[c]{Avg\\w/o u}}                               & \multicolumn{5}{c}{In-domain}                                                                                                                                                      & \multicolumn{4}{c}{Out-of-domain}                \\ \cmidrule(l){5-9} \cmidrule(l){10-13}
\multicolumn{1}{l}{} & \multicolumn{1}{l}{}    & \multicolumn{1}{|l}{} &  & \multicolumn{1}{c}{1p} & \multicolumn{1}{c}{2p} & \multicolumn{1}{c}{3p} & \multicolumn{1}{c}{2i} & \multicolumn{1}{c}{3i} & \multicolumn{1}{c}{ip} & \multicolumn{1}{c}{pi} & \multicolumn{1}{c}{2u} & \multicolumn{1}{c}{up} \\ \midrule
\multirow{8}{*}{\makecell[c]{NELL\\-995}}& \multicolumn{1}{|l|}{GQE~\tohide{hamilton2018embedding}}                                    & 24.8                                   & 27.0                                                & 41.7                   & 23.1                   & 20.3                   & 31.8                   & 45.4                   & 8.1                   & 18.8                   & 20.0                   & 13.9                  \\
                          & \multicolumn{1}{|l|}{Q2B~\tohide{ren2019query2box}}                                       & 30.6                                      & 31.7                                                & 55.5                   & 26.6                   & 23.3                   & 34.3                   & 48.0                   & 13.2                   & 21.2                   & 36.9                   & 16.3                  \\
                          & \multicolumn{1}{|l|}{EmQL~\tohide{sun2021faithful}$^1$}                                   & 27.7                                      & 29.4                                                & 45.6                   & 23.1                   & 17.2                   & 33.1                   & 48.3                   & 14.3                   & 24.4                   & 22.6                   & \underline{20.7}                  \\
                          & \multicolumn{1}{|l|}{BiQE~\tohide{kotnis2021answering}}                                   & \multicolumn{1}{c}{-}                      & 34.4                                                & 58.7                      & 30.5                   & 32.6                   & 37.1                   & \underline{53.1}                   & 10.3                   & 18.7                   & \multicolumn{1}{c}{-}   & \multicolumn{1}{c}{-}  \\
                          %& \multicolumn{1}{|l|}{HypE~\tohide{choudhary2021self}}                                       & 37.1                                      & 37.5                                                &61.8                      & 35.9                   & 31.2                   & 40.0                   & 56.3                   & 14.3                   & 22.7                   & 44.1                   & \bf 27.8                  \\
                          & \multicolumn{1}{|l|}{CQD\footnotesize{(CO)}\normalsize~\tohide{arakelyan2021complex}}     & 36.8                                      & 37.0                                                & \bf 66.7                      & 26.5                   & 22.0                   & \bf 41.0                   & 52.9                   & \underline{19.6}                   & \bf 30.2                   & \bf 53.1                   & 19.4                  \\
                          & \multicolumn{1}{|l|}{CQD\footnotesize{(Beam)}\normalsize~\tohide{arakelyan2021complex}}   & \underline{37.5}                                      & \underline{38.5}                                                & \bf 66.7                   & 35.0                   & 28.8                   & \bf 41.0                   & 52.9                   & 17.1                   & 27.7                   & \bf 53.1                   & 15.6                  \\ \cmidrule{2-13}
                          & \multicolumn{1}{|l|}{\method} & \bf 39.8                                      & \bf 40.6                                                & \underline{62.5}                   & \bf 40.1                   & \bf 36.7                   & \underline{40.5}                   & \bf 54.6                   & \bf 20.3                   & \underline{30.0}                   & \underline{46.9}                   & \textbf{27.0}                  \\ \midrule
\multirow{8}{*}{\makecell[c]{FB15k\\-237}}& \multicolumn{1}{|l|}{GQE~\tohide{hamilton2018embedding}}                                  & 23.0                                      & 25.0                                                & 40.5                   & 21.3                   & 15.3                   & 29.8                   & 41.1                   & 8.5                   & 18.2                   & 16.7                   & 16.0                  \\
                          & \multicolumn{1}{|l|}{Q2B~\tohide{ren2019query2box}}                                       & 26.8                                      & 28.3                                                & 46.7                   & 24.0                   & 18.6                   & 32.4                   & 45.3                   & 10.8                   & 20.5                   & 23.9                   & \underline{19.3}                  \\
                          & \multicolumn{1}{|l|}{EmQL~\tohide{sun2021faithful}$^1$}                                   & 21.9                                 & 24.1                                                & 38.9                           & 20.1                   & 15.4                   & 27.5                   & 38.6                   & 10.1                   & 18.4                           & 11.5                   & 16.5                  \\
                          & \multicolumn{1}{|l|}{BiQE~\tohide{kotnis2021answering}}                                   & -                                          & 29.3                                                & 43.9                   & 28.1                   & 23.9                   & 33.3                   & \underline{47.4}                   & 11.0                   & 17.7                   & -                       & -                      \\
                          %& \multicolumn{1}{|l|}{HypE~\tohide{choudhary2021self}}                                       & \underline{33.5}                                      & \bf 35.9                                                & \bf 57.2                   & \bf 36.6                   & \underline{25.5}                   &\bf  39.9                   & \underline{52.7}                   & 14.5                   & 246                   & 22.5                   &\bf 28.2                  \\
                          & \multicolumn{1}{|l|}{CQD\footnotesize{(CO)}\normalsize~\tohide{arakelyan2021complex}}     & 27.2                             & 29.0                                                & \bf 51.2                   & 21.3                   & 13.1                   & \underline{35.2}                   & 45.7                   & \underline{14.6}                   & 22.2                   & 28.1                   & 13.2                  \\
                          & \multicolumn{1}{|l|}{CQD\footnotesize{(Beam)}\normalsize~\tohide{arakelyan2021complex}}   & \underline{29.0}                             & \underline{31.5}                                                & \textbf{51.2}                   & \underline{28.8}                   & \underline{22.1}                   & \underline{35.2}                   & 45.7                   & 12.9                   & \underline{24.9}                   & \underline{28.4}                   & 12.1                  \\ \cmidrule{2-13}
                          & \multicolumn{1}{|l|}{\method} & \bf 33.6                                     & \textbf{35.7}                                                & \underline{47.9}                   & \textbf{32.3}                   & \bf 27.7                   & \textbf{39.8}                   & \bf 53.9                   & \bf 19.0                   & \bf 29.4                   & \bf29.5                   & \textbf{22.5}                                 \\  
\bottomrule[1.2pt]
\end{tabular}

\tohide{
\midrule
\multirow{8}{*}{FB15k}  & \multicolumn{1}{|l|}{GQE~\cite{hamilton2018embedding}}                                    & 38.4                                      & 40.4                                                & 63.0                   & 346                   & 25.0                   & 51.5                   & 61.1                   & 15.3                   & 32.0                   & 36.2                   & 27.1                  \\
                          & \multicolumn{1}{|l|}{Q2B~\cite{ren2019query2box}}                                       & 48.3                                      & 48.7                                                & 79.0                   & 41.0                   & 30.0                   & 59.0                   & 71.0                   & 21.0                   & 40.0                   & 61.0                   & 33.0                  \\
                          & \multicolumn{1}{|l|}{EmQL~\cite{sun2021faithful}$^1$}                                   & 28.7                                      & 31.6                                                & 41.5                   & 25.0                   & 18.8                   & 39.6                   & 50.8                   & 17.6                   & 27.9                   & 16.6                   & 20.7                  \\
                          & \multicolumn{1}{|l|}{BiQE~\cite{kotnis2021answering}}                                   & \multicolumn{1}{l}{-}                      & \multicolumn{1}{l}{-}                                & \multicolumn{1}{l}{-}   & \multicolumn{1}{l}{-}   & \multicolumn{1}{l}{-}   & \multicolumn{1}{l}{-}   & \multicolumn{1}{l}{-}   & \multicolumn{1}{l}{-}   & \multicolumn{1}{l}{-}   & \multicolumn{1}{l}{-}   & \multicolumn{1}{l}{-}  \\
                          & \multicolumn{1}{|l|}{HypE~\cite{2021Hyperboloid}}                                       & 51.3                                      & 51.4                                                & 80.9                   & 48.6                   & 36.5                   & 59.8                   & 72.8                   & 20.6                   & 40.6                   & 61.0                   & 41.0                  \\
                          & \multicolumn{1}{|l|}{CQD\footnotesize{(CO)}\normalsize~\cite{trouillon2016complex}}     & 57.7                                      & 57.9                                                & 92.0                   & 45.0                   & 19.0                   & 80.0                   & 84.0                   & 34.0                   & 51.0                   & 82.0                   & 32.0                  \\
                          & \multicolumn{1}{|l|}{CQD\footnotesize{(Beam)}\normalsize~\cite{trouillon2016complex}}   & 68.3                                      & 70.9                                                & 92.0                   & 78.0                   & 58.0                   & 80.0                   & 84.0                   & 38.0                   & 66.0                   & 84.0                   & 34.5                  \\ \cmidrule{2-13}
                          & \multicolumn{1}{|l|}{\method} & \\%60.9                                      & 63.4                                                & 89.2                   & 61.7                   & 46.7                   & 73.6                   & 79.7                   & 38.5                   & 54.7                   & 79.5                   & 24.4                                 \\
}

==> tables/mrr_table.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{tabular}{@{}ll|p{0.8cm}<{\centering}p{0.8cm}<{\centering}|p{0.8cm}<{\centering}p{0.8cm}<{\centering}p{0.8cm}<{\centering}p{0.8cm}<{\centering}p{0.8cm}<{\centering}p{0.8cm}<{\centering}p{0.8cm}<{\centering}p{0.8cm}<{\centering}p{0.8cm}<{\centering}@{}}
\toprule[1.2pt]
\multirow{2}{*}{Dataset} & \multirow{2}{*}{Model}    & \multirow{2}{*}{Avg}                      & \multirow{2}{* }{\makecell[c]{Avg\\w.o. u}}                               & \multicolumn{5}{c}{In-domain}                                                                                                                                                      & \multicolumn{4}{c}{Out-of-domain}                \\ \cmidrule(l){5-9} \cmidrule(l){10-13}
\multicolumn{1}{l}{} & \multicolumn{1}{l}{}    & \multicolumn{1}{|l}{} &  & \multicolumn{1}{c}{1p} & \multicolumn{1}{c}{2p} & \multicolumn{1}{c}{3p} & \multicolumn{1}{c}{2i} & \multicolumn{1}{c}{3i} & \multicolumn{1}{c}{ip} & \multicolumn{1}{c}{pi} & \multicolumn{1}{c}{2u} & \multicolumn{1}{c}{up} \\ \midrule
\multirow{8}{*}{NELL995}& \multicolumn{1}{|l|}{GQE}                                    & 0.21                                   & 0.228                                                & 0.311                   & 0.193                   & 0.175                   & 0.273                   & 0.399                   & 0.078                   & 0.168                   & 0.159                   & 0.13                  \\
                          & \multicolumn{1}{|l|}{Q2B}                                       & 0.254                                      & 0.267                                                & 0.413                   & 0.227                   & 0.208                   & 0.288                   & 0.414                   & 0.125                   & 0.193                   & 0.266                   & 0.155                  \\
                          & \multicolumn{1}{|l|}{BiQE}                                   & - & -& -& -& -& -& -& -& -& -& -  \\
                          & \multicolumn{1}{|l|}{HypE}                                       & \underline{0.310}                                      & \underline{0.316}                                                & \underline{0.460}                     & \underline{0.306}                   & \underline{0.279}                   & \underline{0.336}                   & \underline{0.486}                   & \underline{0.135}                   & \underline{0.207}                   & \underline{0.318}                   & \bf 0.264                  \\
                          & \multicolumn{1}{|l|}{CQD\footnotesize{(CO)}\normalsize}     & -                                      & -                                                & -                      & -                   & -                   &  -                   & -                   & - & -                   & -                 & -                  \\
                          & \multicolumn{1}{|l|}{CQD\footnotesize{(Beam)}\normalsize}   & -                                     & -                                                & -          &-                & -                   & -                 & -                   & -                 & -                   & -                & -                \\ \cmidrule{2-13}
                          & \multicolumn{1}{|l|}{\method} &  \bf	0.360   & \bf 0.367  & \bf 0.567 &	\bf 0.358 & \bf	0.333 &\bf	0.357 &	\bf 0.486 &	\bf 0.192 &\bf	0.273 &	\bf 0.416 &	\underline{0.255}         \\ \midrule
\multirow{8}{*}{FB15k-237}& \multicolumn{1}{|l|}{GQE}                                  & 0.203                                      & 0.219                                                & 0.346                   & 0.193                   & 0.145                   & 0.250                   & 0.355                   & 0.086                   & 0.156                   & 0.145                   & 0.151                  \\
                          & \multicolumn{1}{|l|}{Q2B}                                       & 0.235                                      & 0.248                                                & 0.400                   & 0.225                   & 0.173                   & 0.275                   & 0.378                   & 0.105                   & 0.180                   & 0.198                   & 0.178                  \\
                          & \multicolumn{1}{|l|}{BiQE}                                   & -                                          & -                                                & -                   & -                   & -                  & -                   & -                   & -                   & -                   & -                       & -                      \\
                          & \multicolumn{1}{|l|}{HypE}                                       & \bf 0.334                                      & \bf 0.366                                                & \bf 0.490                   & \bf 0.343                   & \underline{0.237}                   & \underline{0.339}                   & \bf 0.440                   &\bf 0.305                   & \bf 0.410                   & \underline{0.186}                   &\bf 0.260                  \\
                          & \multicolumn{1}{|l|}{CQD\footnotesize{(CO)}\normalsize}     & - & -& -& -& -& -& -& -& -& -& -                  \\
                          & \multicolumn{1}{|l|}{CQD\footnotesize{(Beam)}\normalsize}   &  - & -& -& -& -& -& -& -& -& -& -                 \\ \cmidrule{2-13}
                          & \multicolumn{1}{|l|}{\method} &\underline{0.313}                                       & \underline{0.334}                                                & \underline{0.435}                   & \underline{0.316}                   &\bf 0.269                   &\bf 0.364                   & \bf 0.496                   & \underline{0.184}                   & \underline{0.273}                   &\bf 0.266                   & \underline{0.216} \\                               

\bottomrule[1.2pt]
\end{tabular}

==> tables/semistruct_stats.tex <==

\begin{table}[t]
    \centering
    \resizebox{1.0\textwidth}{!}{
    \begin{tabular}{l|ccrrc}
        \toprule
        & \textbf{\#entity types} & \textbf{\#relation types} & \textbf{\#entities} & \textbf{\#relations} & \textbf{avg. degree} \\
        \midrule
        \textbf{\amazont} & 2 & 3 & 1,032,407 & 3,886,603 & 3.0 \\
        \textbf{\magt} & 4 & 4  & 1,872,968 & 19,919,698 & 10.6\\
        \textbf{\primekgt} & 10 & 18 & 129,375 & 8,100,498 & 62.6 \\
        \bottomrule
    \end{tabular}
    }
    \hspace{3pt}
    \caption{Data statistics on the relational structure of the knowledge bases}
    \label{tab:statistics}
\end{table}

